ReDefining Code Comprehension: Function Naming as a Mechanism for Evaluating Code Comprehension

"Explain in Plain English" (EiPE) questions are widely used to assess code comprehension skills but are challenging to grade automatically. Recent approaches like Code Generation Based Grading (CGBG) leverage large language models (LLMs) to generate code from student explanations and validate its equivalence to the original code using unit tests. However, this approach does not differentiate between high-level, purpose-focused responses and low-level, implementation-focused ones, limiting its effectiveness in assessing comprehension level. We propose a modified approach where students generate function names, emphasizing the function's purpose over implementation details. We evaluate this method in an introductory programming course and analyze it using Item Response Theory (IRT) to understand its effectiveness as exam items and its alignment with traditional EiPE grading standards. We also publish this work as an open source Python package for autograding EiPE questions, providing a scalable solution for adoption.

==> tables/long_short.tex <==
\resizebox{\textwidth}{!}{%
  \begin{tabular}{@{}p{0.3\textwidth}p{0.4\textwidth}p{0.3\textwidth}@{}}
    \toprule
    \textbf{Question} & \textbf{Longest Correct Response} & \textbf{Shortest Correct Response} \\
    \midrule
    %\texttt{multiples\_count} & Returns the number of values in list x and that are multiples of the value y & returns the count of multiples in x \\
    \texttt{count\_odd} & count\_num\_of\_val\_not\_divisble\_by\_two & count\_odd \\
    \hline
    \texttt{collect\_numbers\_below\_threshold} & check\_if\_value\_is\_less\_than\_t\_and\_return\_value & smaller\_values \\
    \hline
    %\texttt{copy\_until\_negative} & A function that makes a list of the negative numbers in the list x, that come before the first positive number & returns the first positive number in the list \\
    %\hline
    \texttt{abs\_list\_values} & if\_value\_of\_index\_is\_negative\_return\_it\_as\_positive & make\_positive \\
    \hline
    %\texttt{replace\_x\_with\_z} & change the value of the element in the list that has the same value as the value of y to z & replaces integer y with z in list \\
    %\hline
    %\texttt{count\_occurrences\_case\_insensitive} & it returns the count of the amount of times string y appears in string x, no matter if it is upper or lowercase & count the number of string in the given list regardless the case \\
    %\hline
    \texttt{count\_string\_length} & count\_how\_many\_strings\_length\_is\_equal\_to\_n & count\_strings \\
    \bottomrule
\end{tabular}}

